Dictionary Learning by Dynamical Neural Networks

A dynamical neural network consists of a set of interconnected neurons that interact over time continuously. It can exhibit computational properties in the sense that the dynamical system's evolution and/or limit points in the associated state space can correspond to numerical solutions to certain mathematical optimization or learning problems. Such a computational system is particularly attractive in that it can be mapped to a massively parallel computer architecture for power and throughput efficiency, especially if each neuron can rely solely on local information (i.e., local memory). Deriving gradients from the dynamical network's various states while conforming to this last constraint, however, is challenging. We show that by combining ideas of top-down feedback and contrastive learning, a dynamical network for solving the l1-minimizing dictionary learning problem can be constructed, and the true gradients for learning are provably computable by individual neurons. Using spiking neurons to construct our dynamical network, we present a learning process, its rigorous mathematical analysis, and numerical results on several dictionary learning problems.

==> background_tang.tex <==
\section{Background}


%In this paper we use a network of spiking neurons to realize our dynamical neural
%network. This section describes the model of these neurons, derives the dynamics and
%key properties of the network, and shows how to configure it to perform
%sparse coding.

\subsection{Integrate-and-Fire Neuron Model and Network Dynamics}
\label{sec:neuron_model}

An integrate-and-fire neuron has two internal state variables that govern its dynamics: 
the \textit{current} $\curr(t)$
and the \textit{potential} $\poten(t)$.
The key output of a neuron is a time sequence of spikes -- spike train -- that it produces.
A neuron's spike train is generated by its potential $\poten(t)$; $\poten(t)$ is
in turn driven by the current $\curr(t)$, which is in turn driven by a 
\textit{constant bias} $\bias$ (bias in short) and the spike trains of other neurons
to which it is connected. Specifically, each neuron has a configured firing threshold
$\thres > 0$. When $\poten(t)$ reaches $\thres$, say at time $t_k$, a spike 
given by the Dirac delta function $\spike(t-t_k)$ is generated and $\poten(t)$ is 
reset to 0: $\poten(t_k^+) = 0$. For
$t > t_k$ and before $\poten(t)$ reaches $\thres$ again, $\poten(t) = \int_{t_k}^t \curr(s)\,ds$.

In a system of $N$ neurons $n_i$, $i=1,2,\ldots,N$, 
let
$\spiketrain_j(t) = \sum_k \spike(t-t_{j,k})$ 
denote the spike train of neuron $n_j$. 
The current $\curr_i(t)$ of $n_i$ is given in terms of
its bias $\bias_i$ and the spike trains $\{\spiketrain_j(t)\}$: 
\begin{equation}
\label{eqn:soma_current}
\textstyle \curr_i(t) = \bias_i + \sum_{j\neq i} W_{ij}\,(\alpha \ast \spiketrain_j)(t),
\end{equation}
where $\alpha(t) = \frac{1}{\tau}e^{-t/\tau}$ for $t\ge 0$, $\alpha(t) = 0$ for $t < 0$ and
$\ast$ is the convolution operator. Neuron $n_j$ inhibits (excites) $n_i$ if $W_{ij} < 0$
($W_{ij} > 0$). If $W_{ij} = 0$, neurons $n_i$ and $n_j$ are not connected.
For simplicity, we consider
only $\tau=1$ throughout the paper.

%As a computational model, each neuron evolves in parallel and asynchronously.
%One-sided communication in the form of a one-bit signal from Neuron $n_j$
%to Neuron $n_i$ occurs only if the two are connected and only when the former
%spikes. Each neuron only stores its internal states and one row of the $W$ matrix.
%That this model can potentially be realized in a power-efficient and massively parallel
%implementation makes spiking neural networks and thus dynamical neural networks in general
%valuable to the research community.

%In the simplest case when none of the neurons are inter-connected and $\poten_i(0) < \thres_i$
%for all $i$, then $\curr_i(t) = \bias_i$ for all $i$ and all $t \ge 0$. Hence those
%neurons $n_i$ with $\bias_i > 0$ produces a spike train of constant inter-spike interval 
%of $\thres_i/\bias_i$; those neurons with $\bias_i \le 0$ will have no spiking activities.
%When however the neurons are inter-connected, the dynamics becomes non-trivial. It turns
%out that one can so describe the dynamics mathematically that useful properties
%related to the current and spike train can be derived. Consequently, a network of spiking
%neurons can be configured to help solve certain practical problems.


%\subsection{Dynamics, Trajectories, and Limit Points}
%\label{sec:dynamics}

%Given a system of $N$ neurons $n_i$, $i=1,2,\ldots,N$, we use vector notations
%$\currvec(t)$ and $\spiketrainvec(t)$ to denote the $N$ currents and spike trains.
%The vector $\biasvec$ and $\thresvec$ are the input biases and firing thresholds.
%The convolution $(\alpha\ast\spiketrainvec)(t)$ is the $N$-vector whose
%$i$-th component is $(\alpha\ast\spiketrain_i)(t)$. For simplicity, we consider
%only $\tau=1$ throughout the paper. Thus $\alpha(t) = e^{-t}$ for $t\ge 0$ and 0 otherwise. 
%Equation~\ref{eqn:soma_current}
%in vector form is
%\begin{equation}
%\label{eqn:vector_soma_current}
%\currvec(t) = \biasvec + W (\alpha\ast\spiketrainvec)(t)
%\end{equation}
%where $W\in\reals^{N\times N}$ and $W_{ii}=0$, encodes the inhibitory/excitatory 
%connections among the neurons. 

%Because 
%$\frac{d}{dt} (\alpha\ast\spiketrain)(t) = \spiketrain(t)-(\alpha\ast\spiketrain)(t)$,
%we have
%\begin{equation}
%\label{eqn:current_dot}
%\dot{\currvec}(t) = \biasvec - \currvec(t) + W\cdot\spiketrainvec(t).
%\end{equation}

The network dynamics can studied via the filtered quantities of average current and spike rate, defined respectively as,
\begin{equation}
\label{eqn:avgcur_spikerate_def}
\avgcurrvec(t) \bydef \frac{1}{t}\int_0^t \currvec(s)\,ds, \qquad
\spikeratevec(t) \bydef \frac{1}{t}\int_0^t \spiketrainvec(s)\,ds.
\end{equation}
We use vector notations
$\currvec(t)$ and $\spiketrainvec(t)$ to denote the $N$ currents and spike trains.
%Filtering Equation~\ref{eqn:current_dot} yields
%\begin{align}
%\dot{\avgcurrvec}(t) &= 
%\biasvec - \avgcurrvec(t) + W\,\spikeratevec(t) + (\currvec(0)-\avgcurrvec(t))/t \nonumber \\
%\avgcurrvec(t)-\Thres \,\spikeratevec(t) &=
%\biasvec + (W-\Thres)\,\spikeratevec(t) \nonumber \\
% &\phantom{kk}
%   + (\currvec(0)-\avgcurrvec(t))/t - \dot{\avgcurrvec}(t)
%\label{eqn:avgcurr_spikerate_dynamics}
%\end{align}
%where $\Thres = {\rm diag}(\thresvec)$. The following has been established
%previously in~\cite{shapero2014optimal} and~\cite{tang2016sparse} under the assumption that
%$\Maxnorm{\currvec(t)}\le C$ for all $t\ge 0$ for some $C > 0$.
%\begin{mythm}
%\label{thm:basic_limits}
%As $t\tendsto \infty$,
%$\dot{\avgcurrvec}(t)$, 
%$\frac{1}{t}(\currvec(0)-\avgcurrvec(t))$ and
%$\max(\avgcurrvec(t),\vvzero)-\Thres\,\spikeratevec(t)$
%all converge to $\vvzero$. In particular,
%$(\avgcurrvec(t)-\Thres\,\spikeratevec(t)) -
%(\biasvec + (W-\Thres)\,\spikeratevec(t))$
%converges to $\vvzero$.
%\end{mythm}
%Applying Theorem~\ref{thm:basic_limits} to Equation~\ref{eqn:avgcurr_spikerate_dynamics}
%yields the following.
%\begin{mythm}
%\label{thm:trajectory_large_time}
%Given any $\epsilon > 0$, there exists $T > 0$ such that for all $t>T$,
%\[
%\Maxnorm{ (\avgcurrvec(t)-\Thres\,\spikeratevec(t)) -
%(\biasvec + (W-\Thres)\,\spikeratevec(t)) } < \epsilon.
%\]
%\end{mythm}
The following theorem characterizes limit points of the trajectory $(\avgcurrvec(t),\spikeratevec(t))$.
%Recall that $(\avgcurrvec^*,\spikeratevec^*)$ is a limit point if given any $\epsilon > 0$,
%there exists a time $T > 0$ large enough such that $(\avgcurrvec(T),\spikeratevec(T))$ is within
%$\epsilon$ to $(\avgcurrvec^*,\spikeratevec^*)$.
\begin{mythm}
\label{thm:limit_points}
Given any limit point $(\avgcurrvec^*,\spikeratevec^*)$, 
we must have 
$\biasvec + (W - \Thres)\,\spikeratevec^* \le \vvzero$, $\spikeratevec^*\,\odot\, (\biasvec + (W - \Thres)\,\spikeratevec^*) = \vvzero$ and 
$\spikeratevec^* \ge 0$,
where $\odot$ is the elementwise product.
\end{mythm}
The vector $\biasvec$ and $\thresvec$ are the input biases and firing thresholds, and $\Thres = {\rm diag}(\thresvec)$.
$W\in\reals^{N\times N}$ and $W_{ii}=0$, encodes the inhibitory/excitatory 
connections among the neurons. 
Establishing Theorem~\ref{thm:limit_points} is straightforward using known characteristics of the average current and spike rate studied in ~\cite{shapero2014optimal} and~\cite{tang2016sparse}. We relegate all proofs to the Appendix.
%%PROOF
%\begin{myproof}
%Theorem~\ref{thm:basic_limits} shows that
%$\avgcurrvec^* - \Thres\,\spikeratevec^* \le \vvzero$ and the
%elementwise product
%$\spikeratevec^*\,\odot\, (\avgcurrvec^* - \Thres\,\spikeratevec^*) = \vvzero$.
%But Equation~\ref{eqn:avgcurr_spikerate_dynamics} shows that
%$
%\avgcurrvec^* - \Thres\,\spikeratevec^*  = 
%\biasvec + (W - \Thres)\,\spikeratevec^*
%$
%and the theorem here is established. \qed
%\end{myproof}


\subsection{Non-negative Sparse Coding}
\label{sec:non-negative-sparse-coding}


Given a non-negative dictionary $D\in\reals_{\ge 0}^{M\times N}$,
a positive 
scaling vector $\vvs = [s_1,s_2,\ldots,s_N]^T\in\reals_{>0}^N$ and
an image $\vvx\in\reals_{\ge 0}^M$,
the non-negative sparse coding problem can be formulated as
\begin{equation}
\textstyle \vva^* = \argmin_\mathbf{\vva \geq \vvzero} 
l\left(\vva\right), 
l(\vva)=
\frac{1}{2}\Enormsq{ \vvx - D\,\vva } +
\lambda\,\Onenorm{ S\,\vva }
\label{eqn:nn_lasso}
\end{equation}
where $S={\rm diag}(\vvs)$.
Using the well-known KKT condition in optimization theory \cite{BoydVandenberghe04},
$\vva^*$ is an optimal solution iff there exists a slack variable $\vve^*\in\reals^N$ such that
all of the following hold:
%\begin{align}
%\left\{\begin{matrix}
%&\vvzero \in \partial l(\vva^*) - \vve^* & (\textrm{stationarity}) \\
%&\vve^* \odot \vva^* = \vvzero & (\textrm{complementarity})\\
%&\vva^* \ge \vvzero, \vve^* \ge \vvzero & (\textrm{feasibility})
%\end{matrix}\right.
%\label{eq:kkt_sc}
%\end{align}
\begin{equation}
\vvzero \in \partial l(\vva^*) - \vve^* \; (\textrm{stationarity}), \;
\vve^* \odot \vva^* = \vvzero \; 
 (\textrm{complementarity}), \;
\vva^* \ge \vvzero, \vve^* \ge \vvzero \; (\textrm{feasibility}),
\nonumber
\end{equation}
where $\partial l$ is the generalized gradient of $l$. 
%Note that the generalized gradient $\partial l(\vva)$ is
%$D^T D\vva - D^T \vvx + \lambda \vvs \odot \partial \Onenorm{\vva}$
%and that $\partial |a_i| = 1$ when $a_i > 0$ and 
%equals the interval $[-1,1]$ when $a_i = 0$.
Straightforward derivation then shows that
$\vva^*$ is an optimal solution iff
\begin{equation}
\label{eqn:applied_kkt}
\begin{aligned}
%\vvzero & \ge D^T\,\vvx - \lambda\,\vvs - D^T D \vva^* \;{\rm and}\\
%\vva^*\,\odot\,
%\vvzero & = (D^T\,\vvx - \lambda\,\vvs - D^T D \vva^*).
D^T\,\vvx - \lambda\,\vvs - D^T D \vva^* \  \le  \vvzero\ ;{\rm \phantom{kk} and \phantom{kk}}
\vva^*\,\odot\, 
(D^T\,\vvx - \lambda\,\vvs - D^T D \vva^*)  = \vvzero.
\end{aligned}
\end{equation}
Note the similarity between Equation~\ref{eqn:applied_kkt} and Theorem~\ref{thm:limit_points}.
We now use this observation to configure a $N$-neuron system depicted in Figure~\ref{fig:networks}(a)
so as to solve Equation~\ref{eqn:nn_lasso}.
Set $\thresvec = {\rm diag}(D^T D)$ as the firing thresholds and set
$\biasvec = D^T\vvx - \lambda\vvs$ as the bias.
Define the inhibition matrix to be $-(D^T D - \Thres)$,
$\Thres = {\rm diag}(\thresvec)$. Thus neuron-$j$ inhibits
neuron-$i$ with weight $-\vvd_i^T \vvd_j \le 0$. 
%In this configuration,
%it is easy to establish $\Maxnorm{\currvec(t)} \le C$ for all 
%$t\ge 0$ for some $C > 0$ as all connections are inhibitions. 
From Theorem~\ref{thm:limit_points}, any limit point $(\avgcurrvec^*,\spikeratevec^*)$
of the trajectory $(\avgcurrvec(t),\spikeratevec(t))$ satisfies 
$\biasvec+(W-\Thres)\spikeratevec^* \le \vvzero$ and
$\spikeratevec^*\,\odot\, (\biasvec+(W-\Thres)\spikeratevec^* )  = \vvzero$.
But $\biasvec = D^T\vvx - \lambda\,\vvs$ and
$W-\Thres = -D^T D$. Thus $\spikeratevec^*$ solves 
Equation~\ref{eqn:nn_lasso}. And in particular, if the solution to
Equation~\ref{eqn:nn_lasso} is unique, the trajectory can only have one
limit point, which means in fact the trajectory converges to the sparse
coding solution.
This result can be easily extended to the network in Figure~\ref{fig:networks}(b) by expanding the bias into another layer of input neuron with $F=D^T$.

%This recently established result on sparse coding (\cite{tang2016sparse} and
%\cite{shapero2014optimal}) motivates us to explore the natural follow-on
%question of dictionary learning. To this end, we devised a new topology
%shown in Figure~\ref{fig:networks}(b) where (1) the dictionary will be stored
%explicitly as synaptic weights and (2) excitatory connections in the form of
%feedback are added. The next section details this network's working.



==> learning.tex <==


\section{Dictionary Learning}
\label{sec:learning}
In dictionary learning, we are given $P$ images $\ssup{\vvx}{p}\in\reals_{\ge0}^M$, 
$p=1,2,\ldots,P$.  
The goal is to find a dictionary consisting of a prescribed number of $N$ atoms,
$D = [\vvd_1,\vvd_2,\ldots,\vvd_N]$, $D \in \reals^{M\times N}$ such that each of
the $P$ images can be sparsely coded in $D$. We focus here on non-negative
dictionary and formulate our 
minimization problem as
\begin{equation}
\label{eqn:dictionary_learning}
\argmin_{\ssup{\vva}{p} \ge \vvzero,
D \ge \vvzero}
\sum_{p=1}^P l(D,\ssup{\vvx}{p},\ssup{\vva}{p}), \textrm{\phantom{k}}
l(D,\vvx,\vva) = \frac{1}{2}\Enormsq{\vvx - D\vva} + \lambda_1 \Onenorm{S\vva}
+ \frac{\lambda_2}{2} \Fnormsq{D},
\end{equation}
$S$ being a positive diagonal scaling matrix.
%%In our dynamical network, 
%%Equation~\ref{eqn:dictionary_cost} works better 
%%compared to the somewhat common formulation 
%%that replaces the penalty term $\Fnormsq{D}$ by 
%%explicit constraints on the size of $D$, 
%%such as, each atom $\vvd_i$ to have norm no bigger than 1. 

Computational methods such as stochastic online training~\cite{aharon2008sparse}
%and~\cite{mairal2009online}
is known to be effective
for dictionary learning. With this method, one iterates on the following two steps,
starting with a random dictionary.
\begin{enumerate}
\item Pick a random image $\vv{x} \leftarrow \ssup{\vv{x}}{p}$ and obtain
sparse code $\vv{a}$ for the current dictionary $D$ and image $\vv{x}$.
\item Use gradient descent to update $D$ with a learning rate $\eta$. The 
gradient $\nabla_D$ with respect to $D$ is in a simple form and the update
of $D$ is 
\begin{equation}
\label{eqn:update_D}
D^{({\rm new})} \leftarrow
D - \eta \left((D\vv{a}-\vv{x})\vv{a}^T + \lambda_2 D \right).
\end{equation}
\end{enumerate}
The above stochastic gradient consists a reconstruction term, $D\vv{a}$, which requires connection weights that encode $D$ to compute. However, a feedforward-only network topology only has weights $F=D^T$, making this term uncomputable. 
To address this issue, we explicitly introduce feedback weights $B$ to represent $D$, as shown in Figure~\ref{fig:networks}(c). The strength of feedback is controlled by a scalar parameter $0 \le \gamma < 1$ 
that will be varied during the learning process. The parameter $\gamma$ also controls the magnitude of bias current to all neurons in the network.
Note that when $\gamma=0$, the network is reduced to Figure~\ref{fig:networks}(b).
%We now explain how the dynamical network in Figure~\ref{fig:networks}(b)
%can perform the computations just outlined.

%The figure shows two ``layers'' of neurons.
%The lower layer consists of $M$ neurons we call input neurons, $n_{I,i}$
%for $i=1,2,\ldots,M$; the upper layer consists of $N$ neurons we call
%coding neurons $n_{C,i}$ for $i=1,2,\ldots,N$. 

%Each coding neuron $n_{C,i}$ receives excitatory signals from all the
%input neurons $n_{I,j}$ with a weight of $F_{ij} \ge 0$. That is, each
%coding neuron has a row of the matrix $F \in \reals_{\ge 0}^{N\times M}$.
%In addition, neuron $n_{C,i}$ receives inhibitory signals from all other
%coding neurons $n_{C,j}$ with weight $-W_{ij} \le 0$. 
%%We use $W$ to denote
%$W$ denotes
%this matrix of weights: $W\in\reals_{\ge 0}^{N\times N}$ and
%${\rm diag}(W) = \vvzero$.
%The firing thresholds are 
%$\thresvec = [\thres_1,\thres_2,\ldots,\thres_N]^T$ and the matrix
%$W+\Thres$, $\Thres = {\rm diag}(\thresvec)$, appears often and will
%denote it as $H \bydef W + \Thres$.
%Each neuron $n_{C,i}$ also receives a constant negative bias of 
%$-(1-\gamma)\lambda_1 s_i$ where $0 \le \gamma < 1$ is an important parameter
%that will be varied during the learning process to be detailed momentarily.

%Each input neuron $n_{I,i}$, $i=1,2,\ldots,M$, with firing threshold fixed
%to be 1, receives a bias of $(1-\gamma)x_i$. Typically
%$x_i$ corresponds to the $i$-th pixel value of an input image in question
%during the learning process. In addition, it receives excitatory spikes
%from each of the coding neurons with weights $\gamma B_{ij} \ge 0$.
%That is each input neuron has a row of the matrix $B\in\reals_{\ge 0}^{M\times N}$.
%These excitatory signals from the coding neurons constitute 
%the crucial feedback mechanism we devised here that enables dictionary learning.

To make connection with sparse coding, we denote by $(\vv{e}_\gamma(t), \vv{f}_\gamma(t))$ to relate to the ``slack variables'' in the KKT conditions discussed in Section~\ref{sec:non-negative-sparse-coding}, for the coding and input neurons, respectively.
The subscript $\gamma$ denotes the configuration of the tunable parameter $\gamma$ with which the network operates.
\begin{equation}
\label{eqn:block_eqn}
\begin{aligned}
\left[
\begin{matrix}
\vv{e}_\gamma(t) \\
\vv{f}_\gamma(t)
\end{matrix}
\right]
 & \bydef
\left[
\begin{matrix}
\vv{u}_\gamma(t)-\Thres\vv{a}_\gamma(t) \\
\vv{v}_\gamma(t)-\vv{b}_\gamma(t)
\end{matrix}
\right]  =
\left[
\begin{matrix}
-(1-\gamma)\lambda_1\vv{s} \\
(1-\gamma)\vv{x}
\end{matrix}
\right]
+
\left[
\begin{matrix}
-H &  F \\
\gamma B   & -I 
\end{matrix}
\right]
\,
\left[
\begin{matrix}
\vv{a}_\gamma(t)\\
\vv{b}_\gamma(t)
\end{matrix}
\right] 
+
\bb{\Delta}(t)
\end{aligned}
\end{equation}
$(\bb{\mu}(t),\bb{\nu}(t))$, 
$(\vv{u}(t),\vv{v}(t))$ and
$(\vv{a}(t),\vv{b}(t))$ denotes the currents, average currents and
spike rates for the coding and input neurons, respectively.
$H \bydef W + \Thres$ for the simplicity of presentation.
It can be shown that $\bb{\Delta}(t)$ converge to $\vvzero$ as
$t \rightarrow \infty$.

\subsection{Sparse Coding}
\label{sec:sparse_coding}
As discussed in Section~\ref{sec:non-negative-sparse-coding},
existing result shows that sparse coding can be performed with $\gamma=0$,
$F^T=B=D$ and $H=FB=D^T D$. We
extend this result in several aspects: 
(1) $\gamma$ can be set to any values in $[0,1)$,
(2) $H$ needs not be $FB$ exactly; $\|H-FB\|$ being small suffices,
and
(3) as long as $t$ is large enough, $\vv{a}_\gamma(t)$ solves an approximate
sparse coding problem. These are made precise as follows.

\begin{mythm}
\label{thm:perturbation}
Consider the configuration $F^T=B=D$ and $\gamma\in[0,1)$. Suppose the
soma currents and thus spike rates $\Maxnorm{\vv{a}_\gamma(t)}$ are bounded.
Let $H = D^TD + (\lambda_1\oneminus{\gamma})^{-1}\Delta_H$, $\oneminus{\gamma} = 1-\gamma$, be such that
$4\Onenorm{\Delta_H}\Maxnorm{\vv{a}_\gamma(t)} < \min\{s_i\}$.
Then, for any $\epsilon > 0$ there is $T > 0$ such that for all $t>T$,
$\Maxnorm{\vv{a}_\gamma(t)-\perturbed{\vv{a}}(t)} < \epsilon$ and 
$\perturbed{\vv{a}}(t)$ solves Equation~\ref{eqn:nn_lasso} with
$S$ replaced by $\perturbed{S}$ where
$\Maxnorm{S-\perturbed{S}} < \min\{s_i\}/2$.
\end{mythm}
%%PROOF
%\begin{myproof}
%Consider $\tau > 0$ and define 
%the vectors $\perturbed{\vv{a}}(t)$ and
%$\perturbed{\vv{u}}(t)$ for $t\ge 0$ by each of their components:
%\[
%(\perturbed{a}_i(t),\perturbed{u}_i(t)) = \left\{
%\begin{array}{l l}
%(a_{\gamma,i}(t), \thres_i a_{\gamma,i}(t))   & \hbox{if $a_{\gamma,i}(t) \ge \tau$,} \\
%(0,\phantom{kk}  \min(u_{\gamma,i}(t),0))     & \hbox{otherwise,}
%\end{array}
%\right.
%\]
%where $\thresvec$ is the diagonal of $D^T D$. Denote the perturbations
%$\bb{\Delta}_a(t) \bydef \perturbed{\vv{a}}(t)-\vv{a}_\gamma(t)$,
%$\bb{\Delta}_u(t) \bydef \perturbed{\vv{u}}(t)-\vv{u}_\gamma(t)$,
%$\perturbed{\vv{e}}_\gamma(t) \bydef
%\perturbed{\vv{u}}(t) - \Thres\perturbed{\vv{a}}(t)$, and
%$\bb{\Delta}_e(t) \bydef \perturbed{\vv{e}}(t)-\vv{e}_\gamma(t)$.
%This construction of $\perturbed{\vv{u}}(t)$ and $\perturbed{\vv{a}}(t)$
%ensures $\Maxnorm{\bb{\Delta}_a(t)} < \epsilon$,
%$\perturbed{\vv{e}}(t)\le\vvzero$, and
%$\perturbed{\vv{e}}(t)\odot\perturbed{\vv{a}}(t) = \vvzero$.
%Recall that $\max(\vv{u}_\gamma(t),\vvzero)-\Thres\vv{a}_\gamma(t)\rightarrow\vvzero$
%(Theorem~\ref{thm:basic_limits}); 
%thus $\Maxnorm{\bb{\Delta}_u(t)} < 2\tau$ at $t$ large enough.
%
%Next, observe that $\vv{v}_\gamma(t)\ge \vvzero$ always $\bb{\nu}_\gamma(t)\ge\vvzero$ always,
%for any setting $\gamma$ in $[0,1)$. Thus Theorem~\ref{thm:basic_limits} implies
%\begin{equation}
%\label{eqn:limit_of_b}
%\vv{b}_\gamma(t) - [ (1-\gamma)\vv{x}+\gamma B \vv{a}_\gamma(t) ] \rightarrow \vvzero
%\end{equation} as
%$t\rightarrow \infty$.
%From Equation~\ref{eqn:block_eqn}, this implies that
%\[
%\bb{e}_\gamma(t) = 
%\oneminus{\gamma}(D^T\vv{x}-\lambda\vv{s}-D^T D \vv{a}_\gamma(t) - \lambda \Delta_H\vv{a}_\gamma(t) + 
%\bb{\Delta}(t))
%\]
%for some $\bb{\Delta}(t)$ where $\Maxnorm{\bb{\Delta}(t)}\rightarrow 0$. Thus
%\[
%(\oneminus{\gamma})^{-1} \perturbed{\vv{e}}(t) =
%D^T \vv{x} - \lambda \perturbed{\vv{s}} - D^T D \perturbed{\vv{a}}(t)
%\]
%where $\perturbed{\vv{s}} = \vv{s}-(\bb{\eta}(t)+\bb{\zeta}(t))$,
%$\bb{\eta}(t)=\Delta_H \vv{a}_\gamma(t)$ and
%$\bb{\zeta}(t) = 
%\lambda^{-1}(D^TD \bb{\Delta}_a(t) + \bb{\Delta}_e(t)/\oneminus{\gamma} + \bb{\Delta}(t))$.
%By assumption on $\Delta_H$, 
%$\vv{s}-\bb{\eta}(t) > (3/4)\vv{s} > \vvzero$.
%Moreover,$\Maxnorm{\bb{\zeta}(t)}$ can be made arbitrarily small by 
%taking $t$ and $1/\tau$ large enough. Thus there exist 
%$\tau, T > 0$ such that for all $t > T$, $\Maxnorm{\bb{\Delta}_a(t)} < \epsilon$ and
%$\Maxnorm{\perturbed{\vv{s}}(t) - \vv{s}} < \min\{s_i\}/2$, implying in particular 
%$\perturbed{\vv{s}}(t) > \vv{s}/2 > \vvzero$. Finally, note that
%\[
%\perturbed{\vv{a}}(t)\ge\vvzero, \phantom{kk}
%(\oneminus{\gamma})^{-1}\perturbed{\vv{e}}(t)\le\vvzero, \phantom{kk}
%(\oneminus{\gamma})^{-1}\perturbed{\vv{e}}(t)\odot
%\perturbed{\vv{a}}(t) = \vvzero,
%\]
%which shows (recall Equation~\ref{eqn:applied_kkt}) that
%$\perturbed{\vv{a}}(t)$ solves Equation~\ref{eqn:nn_lasso} with
%$S$ replaced by $\perturbed{S}$ and the proof is complete. \qed
%\end{myproof}
The key observation to establish Theorem~\ref{thm:perturbation} is that Equation~\ref{eqn:block_eqn} can be simplified as
\[
\vv{e}_\gamma(t) = 
\oneminus{\gamma}(D^T\vv{x}-\lambda_1\vv{s}-D^T D \vv{a}_\gamma(t) - \lambda \Delta_H\vv{a}_\gamma(t) + 
\bb{\Delta}(t)).
\]
This suggests that as long as $\Delta_H$ and $\bb{\Delta}(t)$ is sufficiently small, the slack variable we need to establish sparse coding can be found as  $(\oneminus{\gamma})^{-1}\vv{e}_\gamma(t)$, and $\gamma=0$ is a special case.
At present, we cannot establish a priori that the currents stay bounded
when $\gamma > 0$. Nevertheless, the theorem is applicable in practice
as long as the observed currents stay bounded by some $C$ for $0\le t \le T$
and $C/T$ is small enough. See Section~\ref{sec:discussions} for further
comments.
%Applying Theorem~\ref{thm:perturbation}, we sparse code by running the network for a long
%enough time and call the obtained states loosely as limiting states and
%denote them by $\tilde{\vv{e}}_\gamma$, $\tilde{\vv{f}}_\gamma$,
%$\tilde{\vv{a}}_\gamma$ and $\tilde{\vv{b}}_\gamma$. 
%While $\tilde{\vv{a}}_\gamma$ corresponds to (approximate) sparse code,
%the other states will be useful in the next steps.
%For reasons to be clear momentarily, we perform sparse coding twice: once
%with $\gamma \gets 0$ and once with $\gamma \gets \kappa > 0$ for some
%$\kappa$. Typically $\kappa = 0.7$.

\subsection{Dictionary Adjustment}
\label{sec:dictionary_adjustment}
To obtain the learning gradients, we run the network for a long enough time to sparse code twice: at $\gamma = 0$ and $\gamma = \kappa > 0$, obtaining
$\tilde{\vv{e}}_\gamma$, 
$\tilde{\vv{f}}_\gamma$, 
$\tilde{\vv{a}}_\gamma$ and 
$\tilde{\vv{b}}_\gamma$  at those two configurations. 
We use tilde to denote the obtained states and loosely call them as limiting states.
Denote $1-\kappa$ by $\oneminus{\kappa}$. 
The relationships between the limiting states in these two configurations can be characterized as follows.
\begin{mythm}
	\label{thm:approx_for_DA}
	Given any $\epsilon > 0$, there is a $T > 0$ such that for all $t, t' > T$,
	\begin{align}
	&
	\Maxnorm{ 
		\kappa(B\vv{a}_\kappa(t') - \vv{x}) - 
		(\vv{b}_\kappa(t')-\vv{b}_0(t))  
	} < \epsilon,
	\label{eqn:limiting_states_b} \\
	&
	\| 
	\oneminus{\kappa} H(\vv{a}_0(t)-\vv{a}_\kappa(t')) -  
	\kappa(H - FB)\vv{a}_\kappa(t')  + 
	(\oneminus{\kappa} \vv{e}_0(t) - \vv{e}_\kappa(t') ) \|_\infty < \epsilon.
	\label{eqn:limiting_states_e}
	\end{align}
\end{mythm}
%%PROOF
%\begin{myproof}
%	Equation~\ref{eqn:limit_of_b} implies that
%	\[
%	\kappa(B\vv{a}_\kappa(t') - \vv{x}) - 
%	(\vv{b}_\kappa(t')-\vv{b}_0(t))  
%	\rightarrow \vvzero
%	\quad \hbox{as $t,t'\rightarrow\infty$},
%	\]
%	establishing Equation~\ref{eqn:limiting_states_b}.
%	From Equations~\ref{eqn:block_eqn} and~\ref{eqn:limit_of_b}
%	\begin{align*}
%	&
%	-\oneminus{\kappa}\lambda\vv{s} - \oneminus{\kappa} H\vv{a}_0(t) + \oneminus{\kappa}F\vv{x}
%	- \oneminus{\kappa}\vv{e}_0(t) \rightarrow \vvzero, \;{\rm and}, \\
%	& 
%	-\oneminus{\kappa}\lambda\vv{s} - H\vv{a}_\kappa(t) + \oneminus{\kappa}F\vv{x} + \kappa FB \vv{a}_\kappa(t) 
%	- \vv{e}_\kappa(t) \rightarrow \vvzero.
%	\end{align*}
%	Equation~\ref{eqn:limiting_states_e} thus follows. \qed
%\end{myproof}
Theorem~\ref{thm:approx_for_DA} can be established from simple derivations following Equation~\ref{eqn:block_eqn} and Theorem~\ref{thm:perturbation}. 
Note that Equation~\ref{eqn:limiting_states_b} encodes the learning gradient we need (recall $B=D$ and $\tilde{\vv{a}}_\kappa$ is the approximate sparse code) %Hence we can update the dictionary $D$ by
\[
D\tilde{\vv{a}}_\kappa - \vv{x}
\approx \kappa^{-1}(\tilde{\vv{b}}_\kappa-\tilde{\vv{b}}_0).
\]
In other words, the spike rate differences at the input layer reflect 
the reconstruction error of the sparse code we just computed.
Following Equation~\ref{eqn:update_D}, this implies that the update to each weight can be approximated from the 
spike rates of the two neurons that it connects, while the two spike rates 
surely are locally available to the destination neuron that stores the weight.
%Each of the coding and input neurons can approximate the entire vector $D\tilde{\vv{a}}_\kappa-\vv{x}$
%as each neuron has access to the spike rates $\tilde{\vv{b}}_0$ and $\tilde{\vv{b}}_\kappa$.
Specifically, each coding neuron has a row of the matrix $F = D^T$; each input neuron has a row of the
matrix $B = D$. These neurons each updates its row of matrix via
\begin{equation}
\label{eqn:update_FB}
\begin{aligned}
F_{ij}^{({\rm new})} 
    & \gets F_{ij} - \eta_D\left( \kappa^{-1} (\tilde{\vv{a}}_\kappa)_i 
         \, (\tilde{\vv{b}}_\kappa-\tilde{\vv{b}}_0)_j + \lambda_2 F_{ij} \right) \\
B_{ij}^{({\rm new})} 
    & \gets B_{ij} - \eta_D\left( \kappa^{-1} (\tilde{\vv{a}}_\kappa)_j 
         \, (\tilde{\vv{b}}_\kappa-\tilde{\vv{b}}_0)_i + \lambda_2 B_{ij} \right)
\end{aligned}
\end{equation}
Note that $F^T=B=D$ is maintained.

Ideally, at this point the $W$ and $\Thres$ stored distributively in the coding neurons 
will be updated to $H^{({\rm new})}$
where
$H^{({\rm new})} = F^{({\rm new})} B^{({\rm new})}$. 
Unfortunately,
each coding neuron only possesses one row of the matrix $F^{({\rm new})}$
and does not have access to any values of the matrix $B^{({\rm new})}$. 
To maintain $H$ to be close to $D^T D$ throughout the learning process, we do the following.
First we aim to modify $H$ to be closer to $FB$ (not 
$F^{({\rm new})} B^{({\rm new})}$) by reducing the cost function
$\phi(H) = \frac{1}{2} \Enormsq{ (H-FB)\tilde{\vv{a}}_\kappa }$. The
gradient of this cost function is
$
\nabla_H \phi = G = (H-FB) \tilde{\vv{a}}_\kappa
\tilde{\vv{a}}^T_\kappa
$
which is computable as follows. Equation~\ref{eqn:limiting_states_e} shows that
$(H-FB)\tilde{\vv{a}}_\kappa$
is approximated by
\[
\kappa^{-1}\left(
\oneminus{\kappa}H(\tilde{\vv{a}}_0-\tilde{\vv{a}}_\kappa) + 
\oneminus{\kappa}\tilde{\vv{e}}_0 - \tilde{\vv{e}}_\kappa\right).
\]
Using this approximation, coding neuron $n_{C,i}$ has the information to compute the $i$-th entry of
$(H-FB)\tilde{\vv{a}}_\kappa$ and hence the $i$-th row of $G$.
We modify $H$ by $-\eta_H G$ where $\eta_H$ is some learning rate. This
modification can be thought of as a catch-up correction because
$F$ and $B$ correspond to the updated values from a previous iteration. Because
the magnitude of that update is of the order of $\eta_D$, we have 
$\|H-FB\|\approx\eta_D$ and $\|G\| \approx \eta_D$.
Thus $\eta_H$ should be bigger than $\eta_D$ lest
$\|\eta_H G\| \approx \eta_H \eta_D$ be too small to be an effective 
correction.
In practice, $\eta_H \approx 15 \eta_D$ works very well.
%($eta_D$ = 0.0137, $eta_H$ = 0.197)

In addition to this catch-up correction, we also 
make correction of $H$ due to the update of $-\eta_D \lambda_2 F$
and $-\eta_D \lambda_2 B$ to $F$ and $B$. These updates
lead to a change of $-2\eta_D FB + O(\eta_D^2)$. Consequently, after
Equation~\ref{eqn:update_FB}, we update $H$ by
\begin{equation}
\label{eqn:update_H}
H_{ij}^{({\rm new})} 
     \gets H_{ij} - \eta_H G_{ij} - 2\eta_D \lambda_2 H_{ij}.
\end{equation}
The pseudocode of the proposed learning algorithm can be found in the Appendix.

%\begin{algorithm}
%\begin{algorithmic}
%\STATE \emph{Initialization:} Pick a random dictionary 
%$D \ge \vvzero$ with atoms of
%unit Euclidean norm. Configure $F\leftarrow D^T$, $B \leftarrow D$,
%$\vv{s}\leftarrow [1,1,\ldots,1]^T$, and $H \leftarrow FB$.
%\REPEAT
%  \STATE 1. \emph{Online input:}
%         Pick a random image $\vv{x}$ from $\{\ssup{\vv{x}}{p}\}$
%  \STATE 2. \emph{Sparse coding:} 
%            Run the network at $\gamma$ equal 0 and
%            $\kappa>0$.
%  \STATE 3. \emph{Dictionary update:} Compute 
%\[ 
%\vv{g}_D = D\tilde{\vv{a}}_\kappa - \vv{x}, \quad
%   \vv{g}_H = (H-FB)\tilde{\vv{a}}_\kappa.
%\]
%   Update $F$, $B$ and $H$ according to Equations~\ref{eqn:update_FB}
%   and~\ref{eqn:update_H}. Project the weights to non-negative quadrant.
%  \STATE 4. \emph{Scaling update:}
%            Set the scaling vector $\vv{s}$ to
%         ${\rm diag}(H)$. This scaling helps maintain each atom
%         of the dictionary to be of similar norms.
%\UNTIL{dictionary is deemed satisfactory}
%\end{algorithmic}
%\caption{Dictionary Learning}
%\label{algo:dictionary_learning}
%\end{algorithm}

\input{discussions}

\input{spike_figures}

